IANN: A Unified Framework for Equivariant InterAtomic Neural Networks with User-Friendly Implementation

Machine-learning interatomic potentials (MLIPs) now approach density functional theory (DFT) accuracy at a fraction of its cost, but the practical benefit is limited by software fragmentation: each state-of-the-art architecture is released as a separate codebase, with its own data format, configuration system, training loop and molecular-dynamics interface. Comparing two architectures on the same dataset, or moving a trained model into a production simulation, therefore requires substantial re-engineering. We introduce IANN (InterAtomic Neural Network), an open-source PyTorch framework that reimplements equivariant graph neural networks - PaiNN, NequIP, MACE, Allegro, EquiformerV2, EquiformerV3 and UMA - behind a unified data object, a unified trainer and a single deployment route, so that the architecture is a one-word change in a configuration dictionary. Forces, stresses and virials are obtained for every architecture from one analytic differentiation of the energy with respect to the edge vectors of the atomic graph, exact under periodic boundary conditions. Distributed training is configured automatically from the SLURM, PBS or MPI environment, so the same script runs unchanged from a workstation to a multi-node GPU allocation. Self-describing checkpoints serve directly as ASE calculators, as ensembles reporting uncertainties, or as TorchScript models run inside LAMMPS through bundled C++ pair styles with single- and multi-GPU inference. Trained on a common dataset of millions of structures, the architectures can be compared under identical conditions. We further release PaiNN foundation models trained on 41.9 million curated DFT structures from MPtrj, Alexandria, OMat24, MatPES, OC20, OC22, OC25, MPr2SCAN and MatPESr2SCAN, spanning the PBE, RPBE and r2SCAN functionals. Additionally, IANN provides an agent interface to facilitate integration with autonomous agents.

==> latexmkrc <==
# Build layout
# ------------
# Auxiliary files go to output/, the two PDFs stay beside the sources, so the
# working directory holds only sources plus Manuscript.pdf and SI.pdf.
$aux_dir = 'output';
$out_dir = '.';

# SyncTeX, for ctrl/cmd-click between the PDF viewer and the source. latexmk
# does not pass -synctex=1 on its own, so it has to be requested here.
$pdflatex = 'pdflatex -synctex=1 %O %S';

# xr cross-references into the SI
# ------------------------------
# Manuscript.tex has \myexternaldocument{SI}, which prints the SI's section
# numbers (Section S2, S3, ...) by reading SI.aux. It never compiles the SI
# itself, and nothing else does either: Overleaf builds only the main document.
# Without the rule below those references come out as "??".
#
# The stock version of this rule could not be reconciled with $aux_dir: it ran
# a bare `latex SI`, which drops SI.aux in the working directory, while latexmk
# expects the rule's destination inside the aux directory -- hence the old
# "return code -1" and exit 12. Passing -output-directory puts the file exactly
# where latexmk looks for it, and the two settings then coexist.
#
# latexmk still insists on seeing the rule's destination at ./SI.aux, whatever
# $aux_dir says, and reports "return code -1" (exit 12) without it even though
# every output file is correct. So the pass writes into output/ and the .aux
# alone is lifted beside the sources. That one file is also what xr reads,
# since kpathsea searches the working directory and not output/. It is the
# only build artifact left in the source tree, and .gitignore covers it.
#
# One pdflatex pass, not the customary three plus biber: the manuscript refers
# to the SI only with \ref, which needs section numbers, and those are settled
# after a single pass -- no page numbers, no citations are taken across.
# -draftmode suppresses the PDF, so this does not spend time writing the SI's
# ~9.5 MB of figures on every manuscript compile, which matters against
# Overleaf's compile timeout.
#
# The guard keeps the rule from recursing when the SI is itself the root
# document, in which case latexmk is already building it properly.
add_cus_dep('tex', 'aux', 0, 'makeexternaldocument');
sub makeexternaldocument {
    return if $root_filename eq $_[0];
    system("pdflatex -draftmode -interaction=nonstopmode "
           . "-output-directory=$aux_dir \"$_[0]\"");
    system("cp -f \"$aux_dir/$_[0].aux\" \"$_[0].aux\"");
}

